Circuits and Systems for Embodied AI: Exploring uJ Multi-Modal Perception for Nano-UAVs on the Kraken Shield

Embodied artificial intelligence (AI) requires pushing complex multi-modal models to the extreme edge for time-constrained tasks such as autonomous navigation of robots and vehicles. On small form-factor devices, e.g., nano-sized unmanned aerial vehicles (UAVs), such challenges are exacerbated by stringent constraints on energy efficiency and weight. In this paper, we explore embodied multi-modal AI-based perception for Nano-UAVs with the Kraken shield, a 7g multi-sensor (frame-based and event-based imagers) board based on Kraken, a 22 nm SoC featuring multiple acceleration engines for multi-modal event and frame-based inference based on spiking (SNN) and ternary (TNN) neural networks, respectively. Kraken can execute SNN real-time inference for depth estimation at 1.02k inf/s, 18 {\mu}J/inf, TNN real-time inference for object classification at 10k inf/s, 6 {\mu}J/inf, and real-time inference for obstacle avoidance at 221 frame/s, 750 {\mu}J/inf.

==> src/Data_Acquisition.tex <==
\section{Data Acquisition}
Kraken's unique capability is acquiring data from event-based sensors at very high throughput. We characterized Kraken's I/O subsystem latency for event acquisition from the DVS. In our experimental setup, Kraken was connected to an IniVation DVS132. Multiple event frames were recorded during a 1 second time window, and the acquisition latency was logged using a timer. Repeated acquisitions allowed to span a wide range of event-frames ranging from 1 to 132x104/4 events, the maximum number produced by the DVS camera. These frames were ordered by the number of events to correlate the frame latency versus the number of events. The event-frame request rate was set to 300 event frames per second to not saturate the DVSI input bandwidth in case of DVS maximum activity (104x132 active events). 

==> src/cluster_soa.tex <==
\begin{table}[htb]
\renewcommand{\arraystretch}{1.2}
\begin{minipage}{\textwidth}
\resizebox{\textwidth}{!}{% Resize table to fit the text width while keeping the aspect ratio
\begin{tabular}{@{}lccccccc@{}}
\toprule
                                                                                       & \begin{tabular}[c]{@{}c@{}}VEGA\\ (2022)~\cite{rossiVegaTenCoreSoC2022}\end{tabular}                            & \begin{tabular}[c]{@{}c@{}}DIANA\\ (2023)~\cite{houshmandDIANAEndtoEndHybrid2023}\end{tabular}                                & \begin{tabular}[c]{@{}c@{}}MARSELLUS\\ (2023)~\cite{contiMarsellusHeterogeneousRISCV2024}\end{tabular}                              & \begin{tabular}[c]{@{}c@{}}Chang et. al\\ (2022)~\cite{chang40nm6064TOPS2022}\end{tabular}               & \begin{tabular}[c]{@{}c@{}}Zhang et al.\\ (2022)~\cite{zhang22nm5TOPSFlexible2022}\end{tabular} & \begin{tabular}[c]{@{}c@{}}SIRACUSA\\ (2023)~\cite{prasadSiracusa16Nm2023}\end{tabular}                                       & \textbf{\begin{tabular}[c]{@{}c@{}}KRAKEN \\ PULP Cluster\end{tabular}}          \\ \midrule
\textbf{Technology}                                                                    & 22nm FDX                                                                         & 28nm CMOS                                                                             & 28nm CMOS                                                                               & 22nm FDX                                                                    & 22nm                                                          & 16nm FinFET                                                                                     & 22nm FDX                                                                         \\ \midrule
\textbf{Application}                                                                   & \begin{tabular}[c]{@{}c@{}}IoT GP +\\ DNN SoC\end{tabular}                       & AI-IoT SoC                                                                            & \begin{tabular}[c]{@{}c@{}}IoT GP + \\ AI-IoT SoC\end{tabular}                          & Edge AI ASIC                                                                & \begin{tabular}[c]{@{}c@{}}GP + \\ DNN Robot SoC\end{tabular} & XR SoC                                                                                          & GP + DNN SoC                                                                     \\ \midrule
\textbf{Cores}                                                                         & \begin{tabular}[c]{@{}c@{}}10× RV32IMCFXpulp +\\ Convolution Engine\end{tabular} & \begin{tabular}[c]{@{}c@{}}1× RV32IMCFXpulp +\\ digital NE +\\ AIMC SRAM\end{tabular} & \begin{tabular}[c]{@{}c@{}}1× RV32IMCFXpulp +\\ 16× RV32IMCFXpulpnn +\\ NE\end{tabular} & \begin{tabular}[c]{@{}c@{}}1× 1× Cortex-M3 +\\ MAC Array\end{tabular}       & \begin{tabular}[c]{@{}c@{}}Cortex-M33 +\\ NVPU\end{tabular}   & \begin{tabular}[c]{@{}c@{}}256 KiB (L1) +\\ 2 MiB (L2) +\\ 4 MiB (SRAM)\end{tabular}            & \begin{tabular}[c]{@{}c@{}}1× RV32IMCFXpulp +\\ +8× RV32IMCFXpulpnn\end{tabular} \\ \midrule
\textbf{On-chip SRAM}                                                                  & \begin{tabular}[c]{@{}c@{}}128 KiB (L1)\\ 1600 KiB (L2)\end{tabular}             & 896 KiB(in/out+weights)                                                               & \begin{tabular}[c]{@{}c@{}}128 KiB (L1)\\ 1024 KiB (L2\end{tabular}                     & 768 KiB                                                                     & 1428 KiB                                                      & 4 MiB MRAM (L1)                                                                                 & \begin{tabular}[c]{@{}c@{}}128 KiB (L1)\\ 1 MiB (L2)\end{tabular}                \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}INT\\ Precision\end{tabular}}                       & 8, 16, 32                                                                        & 2, 4, 8, 16, 32                                                                       & \begin{tabular}[c]{@{}c@{}}2, 4, 8, 16, 32 (RISC-V)\\ 2-8 (RBE)\end{tabular}            & \begin{tabular}[c]{@{}c@{}}1, 4, 8 (MAC Array)\\ 32 (Cortex-M3\end{tabular} & 16                                                            & \begin{tabular}[c]{@{}c@{}}2, 4, 8, 16, 32 (RISC-V)\\ 2-8b W, 8b in/out (N-EUREKA)\end{tabular} & 2, 4, 8, 16, 32                                                                  \\ \midrule
\textbf{Supply Voltage {[}V{]}}                                                        & 0.5 - 0.8                                                                        & 0.5 - 0.9                                                                             & 0.5 - 0.8                                                                               & 0.9                                                                         & 0.5 - 1.0                                                     & 0.65 - 0.8                                                                                      & 0.5 - 0.8                                                                        \\ \midrule
\textbf{Max Frequency {[}MHz{]}}                                                       & 450                                                                              & 320                                                                                   & 420                                                                                     & 200                                                                         & 190                                                   & 360                                                                                             & 330                                                                              \\ \midrule
\textbf{Power Range}                                                                   & 1.7 uW - 49.4 mW                                                                 & 10mW - 129 mW                                                                         & 12.8 mW - 123 mW                                                                        & 2.6 mW - 131 mW                                                             & 468 uW - 158 mW                                               & 151 mW - 332 mW                                                                                 & 2mW - 300 mW                                                                     \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}8-bit Peak \\ Performance {[}GOp/s{]}\end{tabular}} & 32.2                                                                             & 140 (NE)\footnote{\label{note1} Value measured for the accelerator engine.}                                                                              & 90\footnoteref{note1}                                                                                      & --                                                                          & \begin{tabular}[c]{@{}c@{}}146\footnoteref{note1} \\ (16b in/W)\end{tabular}     & 698\footnoteref{note1}                                                                                             & 21.5                                                                          \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}8-bit Peak\\ Efficiency {[}TOp/s/W{]}\end{tabular}} & 1.3\footnoteref{note1}                                                                              & 2.07\footnoteref{note1}                                                                                  & 1.8\footnoteref{note1}                                                                                     & 0.94\footnoteref{note1}                                                                        & \begin{tabular}[c]{@{}c@{}}0.7\footnoteref{note1} \\ (16b in/W)\end{tabular}     & 2.68\footnoteref{note1}                                                                                            & 0.38                                                                             \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}Best Peak \\ Performance {[}GOp/s{]}\end{tabular}}  & 32.2                                                                             & \begin{tabular}[c]{@{}c@{}}140 (NE)\\ 29500 (AIMC-SRAM)\end{tabular}                  & \begin{tabular}[c]{@{}c@{}}637\footnoteref{note1}\\ (2b in/W)\end{tabular}                                 & --                                                                          & \begin{tabular}[c]{@{}c@{}}146\footnoteref{note1}\\ (16b in/W)\end{tabular}      & \begin{tabular}[c]{@{}c@{}}19500\footnoteref{note1}\\ (8b in, 2b W)\end{tabular}                                   & \begin{tabular}[c]{@{}c@{}}87\\ (2b in/W)\end{tabular}                           \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}Best Peak\\ Efficiency {[}TOp/s/W{]}\end{tabular}}  & \begin{tabular}[c]{@{}c@{}}1.3\footnoteref{note1}\\ (8b in/W)\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}4.1 (NE, 2b in/W)\\ 600 (AIMC-SRAM)\end{tabular}           & \begin{tabular}[c]{@{}c@{}}12.4\footnoteref{note1}\\ (2b in/W)\end{tabular}                                & \begin{tabular}[c]{@{}c@{}}60.64\footnoteref{note1}\\ (1b in/W)\end{tabular}                   & \begin{tabular}[c]{@{}c@{}}0.7\footnoteref{note1}\\ (16b in/W)\end{tabular}      & \begin{tabular}[c]{@{}c@{}}8.84\footnoteref{note1} \\ (8b in, 2b W)\end{tabular}                                   & \begin{tabular}[c]{@{}c@{}}1.6\\ (2b in/W)\end{tabular}                          \\ \hline
\bottomrule
\end{tabular}
}
\end{minipage}
\caption{State-of-the Art comparison of edge and near-sensor computing systems.}
\label{tab:cluster_soa}
\end{table}

==> src/cutie_soa.tex <==
\begin{table}[htb]
\renewcommand{\arraystretch}{1.2}
\begin{minipage}{\linewidth}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccc}
\hline
& \begin{tabular}[c]{@{}c@{}}Knag et. al\\ (2021)~\cite{knag617TOPSAllDigitalBinary2021}\end{tabular} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Ryu et. al\\ (2023)~\cite{ryuBinarywareHighPerformanceDigital2023}\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Cheon et. al\\ (2023)~\cite{cheon2941TOPSChargeDomain10T2023}\end{tabular}} & \multicolumn{2}{c}{\textbf{\gls{cutie}}}           \\ \hline
\multicolumn{1}{l|}{\textbf{Technology}}                                                              & \multicolumn{1}{c|}{10nm CMOS}                               & \multicolumn{2}{c|}{28nm CMOS}                                                  & \multicolumn{2}{c|}{28nm CMOS}                                                    & \multicolumn{2}{c}{22nm FDX}        \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Computation\\ Method\end{tabular}}}            & \multicolumn{1}{c|}{digital}                                 & \multicolumn{2}{c|}{digital}                                                    & \multicolumn{2}{c|}{digital}                                                      & \multicolumn{2}{c}{digital}         \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Weight \\ Precision\end{tabular}}}             & \multicolumn{1}{c|}{binary}                                  & \multicolumn{2}{c|}{binary}                                                     & \multicolumn{2}{c|}{binary}                                                       & \multicolumn{2}{c}{ternary}         \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Activation\\ Precision\end{tabular}}}          & \multicolumn{1}{c|}{binary}                                  & \multicolumn{2}{c|}{binary}                                                     & \multicolumn{2}{c|}{ternary}                                                      & \multicolumn{2}{c}{ternary}         \\ \hline
\multicolumn{1}{l|}{\textbf{Dataset}}                                                                 & \multicolumn{1}{c|}{CIFAR-10}                                & \multicolumn{2}{c|}{CIFAR-10}                                                   & \multicolumn{2}{c|}{CIFAR-10}                                                     & \multicolumn{2}{c}{CIFAR-10}        \\ \hline
\multicolumn{1}{l|}{\textbf{Accuracy}}                                                                & \multicolumn{1}{c|}{86\%}                                    & \multicolumn{2}{c|}{--}                                                         & \multicolumn{2}{c|}{88.5\%}                                                       & \multicolumn{2}{c}{\textbf{88.6\%}} \\ \hline
\multicolumn{1}{l|}{\textbf{Energy/inf {[}\si{\micro\joule}{]}}}                                                     & \multicolumn{1}{c|}{3.0}                                     & \multicolumn{2}{c|}{3.2}                                                        & \multicolumn{2}{c|}{--}                                                           & \multicolumn{2}{c}{\textbf{2.72}}   \\ \hline
\multicolumn{1}{l|}{\textbf{Core Area {[}\si{\milli\meter}$^2${]}}}                                                     & \multicolumn{1}{c|}{2.1}                                     & \multicolumn{2}{c|}{0.4}                                                        & \multicolumn{2}{c|}{\textbf{0.04}}                                                & \multicolumn{2}{c}{2.96}            \\ \hline
\multicolumn{1}{l|}{\textbf{Throughput {[}TOp/s{]}}}                                                  & \multicolumn{1}{c|}{101}                                     & \multicolumn{1}{c|}{3.4}           & \multicolumn{1}{c|}{\textbf{163}}          & \multicolumn{1}{c|}{2.5}                     & \multicolumn{1}{c|}{--}            & \multicolumn{1}{c|}{16}     & 56    \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Peak\\ Efficiency {[}TOp/s/W{]}\end{tabular}}} & \multicolumn{1}{c|}{86.7}                                    & \multicolumn{1}{c|}{617}           & \multicolumn{1}{c|}{269}                   & \multicolumn{1}{c|}{\textbf{2941}}           & \multicolumn{1}{c|}{943}           & \multicolumn{1}{c|}{1036}   & 446   \\ \hline
\multicolumn{1}{l|}{\textbf{Supply Voltage {[}V{]}}}                                                  & \multicolumn{1}{c|}{0.9}                                     & \multicolumn{1}{c|}{0.37}          & \multicolumn{1}{c|}{0.75}                  & \multicolumn{1}{c|}{0.6}                     & \multicolumn{1}{c|}{1.0}           & \multicolumn{1}{c|}{0.5}    & 0.9   \\ \hline
\bottomrule
\end{tabular}}
\end{minipage}
\caption{State-of-the-Art comparison of \gls{tnn} accelerator engines.}
\label{tab:tnn_soa}
\end{table}

==> src/figures.tex <==
\begin{figure*}
% First row
\vspace{1cm}
% \begin{minipage}[t!]{0.5\linewidth}
%   \begin{center}
%     \includegraphics[width=\linewidth]{figs/kraken_syslevel.png}
%     \caption{System level overview showing the three main computation engines and their integration into the SoC.}
%     \label{fig:syslevel}
%   \end{center}
% \end{minipage}\hfill%
  
% \begin{minipage}[t!]{0.45\linewidth}
%   \begin{center}
%   \includegraphics[width=\linewidth]{figs/application_3.pdf}\\
% %   \vspace{.5cm}
% %     \includegraphics[width=\linewidth]{figs/application.pdf}
%     % \caption{kraken application scenario. events are acquired form the DVS, SNE is activated based on the event-rate. If detection criteria are met, the Cluster and CUTIE are activated. CUTIE run an object classification network on the ROI. Position and object class are sent to the Cluster for object tracking}
%     \caption{Description of the application scenario. The two computation subsystems are shown in red and blue respectively.}
%     \label{fig:application_drone}
%     \end{center}
% \end{minipage}

% \vspace{1cm}
% \begin{minipage}[t!]{0.35\linewidth}
%   \begin{center}
%     \includegraphics[width=0.85\linewidth]{figs/kraken_micrograph.png}
%     \caption{Die micrograph of the Kraken SoC showing the different power domains.}
%     \label{fig:dieshot}
%   \end{center}
% \end{minipage}%
% \hfill
% \begin{minipage}[t!]{.31\linewidth}
%   \begin{center}
%     \includegraphics[width=\linewidth]{figs/kraken_sops_sop_second_watt_large.pdf}
%     \vspace{-0.3cm}
%     \caption{Energy efficiency of the PULP cluster for different bit precision. unless ``fp'' specified, integer arithmetic is indented. SIMD instructions are used below 32bit precision.}
%     \label{fig:cluster}
%   \end{center}
% \end{minipage}
% \hfill%
% \begin{minipage}[t!]{0.33\linewidth}
%     \centering
%     \resizebox{0.75\linewidth}{!}{
%     \begin{tabular}{@{}ll@{}}
%     \toprule
%     Technology & GF \SI{22}{\nano\meter} FDX \\ \midrule
%     Chip area & \SI{9}{\milli\meter\squared} \\ \midrule
%     L2 memory (SRAM) & \SI{1}{\mebi\byte}  \\ \midrule
%     L1 Memory (SRAM) & \SI{128}{\kibi\byte} \\ \midrule
%     VDD Range & \SIrange{0.5}{0.8}{\volt} \\ \midrule
%     Cluster Max. Frequency & \SI{330}{\mega\hertz} \\ \midrule
%     EHWPE Max. Frequency & \SI{330}{\mega\hertz}\\ \midrule
%     FC Max. Frequency & \SI{330}{\mega\hertz} \\ \midrule
%     Power Range & \SIrange{2}{300}{\milli\watt} \\ \bottomrule
%     \end{tabular}%
%     }
%     \caption{Physical implementation details for the kraken chip. Maximum frequency has been measured on 32bit floating point matrix-to-matrix multiplication benchmarks for both FC and cluster. For CUTIE and SNE, CNN workloads have been used.}
%     \label{tab:kraken_details}
% \end{minipage}%
% \begin{minipage}[t!]{0.39\linewidth}
% \includegraphics[width=\linewidth]{figs/staged_inf.pdf}
%     \caption{Application-level power consumption, showing the greatly reduced power consumption in the always-on object-detection mode.}
%     \label{fig:applicationpower}
% \end{minipage}
\vspace{-0.4cm}
% \begin{minipage}[t!]{.5\linewidth}
%     \includegraphics[width=\linewidth]{figs/efficiencyKraken.png}
%     \label{fig:efficiency}
%     \vspace{-1cm}
%     \caption{Comparison of the energy efficiency of the cluster, SNN accelerator and TNN accelerator with state-of-the-art designs.}
% \end{minipage}
\begin{minipage}[t!]{.49\linewidth}
    \includegraphics[width=\linewidth]{figs/soa.pdf}
    % \vspace{-0.5cm}
    \caption{Comparison of the energy efficiency of the cluster, SNN accelerator and TNN accelerator with state-of-the-art designs. In the case of PULP, 2 N-bit OP = 1 N-bit MAC. For CUTIE, 2 ternary OP = 1 ternary MAC. In the case of SNE, 1 SOP = 1 4b-ADD + 1 8b-MUL + 1 8b-COMPARE
  }
    \label{fig:efficiency}
\end{minipage}
\hfill%
\begin{minipage}[t!]{.49\linewidth}
  \begin{center}
    \includegraphics[width=\linewidth]{figs/sne_comb.pdf}
    % \vspace{-0.3cm}
    \caption{SNE inference per second versus the DVS network activity (Top). SNE inference energy versus DVS network activity (Bottom).}
    \label{fig:sne}
  \end{center}
\end{minipage}\hfill%
\end{figure*}







==> src/sne_soa.tex <==
\begin{table}[htb]
\renewcommand{\arraystretch}{1.2}
\begin{minipage}{\linewidth}
\resizebox{\linewidth}{!}{% Resize table to fit the text width while keeping the aspect ratio
\begin{tabular}{lccccccccc}
\hline
                                                                                                      &
                                                                                                      \begin{tabular}[c]{@{}c@{}}SpiNNaker 2\\ (2021)~\cite{hoppnerSpiNNakerProcessingElement2022}\end{tabular} & 
                                                    \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Loihi 2\\ (2022)~\cite{daviesAdvancingNeuromorphicComputing2021}\end{tabular}} &
                                                    \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Tan et. al\\ (2023)~\cite{tan40nm89pJSOP2023}\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Wang et. al\\ (2023)~\cite{wang7pJSOPNeuromorphic2023}\end{tabular}} & \multicolumn{2}{c}{\textbf{\gls{sne}}}           \\ \hline
\multicolumn{1}{l|}{\textbf{Technology}}                                                              &  \multicolumn{1}{c|}{22nm} & \multicolumn{2}{c|}{14nm EUV}                              & \multicolumn{2}{c|}{40nm CMOS}                                                  & \multicolumn{2}{c|}{40nm CMOS}                                                    & \multicolumn{2}{c}{22nm FDX}        \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Neuron Type\end{tabular}}}            & \multicolumn{1}{c|}{Prog}        &          \multicolumn{2}{c|}{Prog}                & \multicolumn{2}{c|}{LIF}                                                    & \multicolumn{2}{c|}{--}                                                      & \multicolumn{2}{c}{ALIF}         \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Neurons\end{tabular}}}             &  \multicolumn{1}{c|}{250}           & \multicolumn{2}{c|}{1000000}                       & \multicolumn{2}{c|}{--}                                                     & \multicolumn{2}{c|}{256$\times$12}                                                       & \multicolumn{2}{c}{8193}         \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Synapses\end{tabular}}}          &  \multicolumn{1}{c|}{20K}        & \multicolumn{2}{c|}{1200000}                          & \multicolumn{2}{c|}{--}                                                     & \multicolumn{2}{c|}{64K$\times$12}                                                      & \multicolumn{2}{c}{18432}         \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Network Type\end{tabular}}} &  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SNN\\ CNN\end{tabular}}    & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}SNN\end{tabular}}                                & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}SNN\\ CNN\end{tabular}}                             & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}SNN\end{tabular}}                     & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}SNN\end{tabular}}         \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Weight\\Precision [bits]\end{tabular}}} &  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Var\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}1-9\end{tabular}}                                    & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}8\end{tabular}}                             & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}5\end{tabular}}                     & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}4\end{tabular}}   \\ \hline
\multicolumn{1}{l|}{\textbf{Supply Voltage {[}V{]}}}                                                                                       & \multicolumn{1}{c|}{0.45 - 0.9} &\multicolumn{1}{c|}{0.75} & \multicolumn{1}{c|}{1.10} &\multicolumn{1}{c|}{0.65}                                     & \multicolumn{1}{c|}{0.9}          & \multicolumn{1}{c|}{0.5}                  & \multicolumn{1}{c|}{0.9}                     & \multicolumn{1}{c|}{0.52} & \multicolumn{1}{c}{0.65}                \\ \hline
\multicolumn{1}{l|}{\textbf{Frequency {[}MHz{]}}}                                                  & \multicolumn{1}{c|}{200} & \multicolumn{2}{c|}{1000} &\multicolumn{1}{c|}{105}                                     & \multicolumn{1}{c|}{259}          & \multicolumn{1}{c|}{12.5}                  & \multicolumn{1}{c|}{100}                     & \multicolumn{2}{c}{85}  \\ \hline
\multicolumn{1}{l|}{\textbf{Power {[}mW{]}}}                                                 &   \multicolumn{1}{c|}{--} & \multicolumn{2}{c|}{--} &\multicolumn{1}{c|}{3.12}                                     & \multicolumn{1}{c|}{12.14}          & \multicolumn{1}{c|}{\textbf{0.5}}                  & \multicolumn{1}{c|}{\textbf{10.26}} & \multicolumn{1}{c|}{17}                     & \multicolumn{1}{c}{46}     \\ \hline
\multicolumn{1}{l|}{\textbf{Performance {[}GSOp/s{]}}}                                                & \multicolumn{1}{c|}{--} & \multicolumn{2}{c|}{--}  & \multicolumn{1}{c|}{1.70}                                     & \multicolumn{1}{c|}{4.15}          & \multicolumn{2}{c|}{--}                     & \multicolumn{1}{c|}{11}     &    \multicolumn{1}{c}{17.9}        \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Operation\\Energy [pJ/SOp]\end{tabular}}}  & \multicolumn{1}{c|}{1700} & \multicolumn{1}{c|}{7.8} & \multicolumn{1}{c|}{--} &\multicolumn{1}{c|}{1.89}                                     & \multicolumn{1}{c|}{2.96}          &\multicolumn{1}{c|}{1.71}                                     & \multicolumn{1}{c|}{4.38}                     &  \multicolumn{1}{c|}{1.5} &  \multicolumn{1}{c}{2.6}     \\ \hline
\end{tabular}}
\end{minipage}
\caption{State-of-the-Art comparison of \gls{snn} accelerator engines.}
\label{tab:sne_soa}
\end{table}
